Visual SLAM: What are the Current Trends and What to Expect?

Vision-based sensors have shown significant performance, accuracy, and efficiency gain in Simultaneous Localization and Mapping (SLAM) systems in recent years. In this regard, Visual Simultaneous Localization and Mapping (VSLAM) methods refer to the SLAM approaches that employ cameras for pose estimation and map generation. We can see many research works that demonstrated VSLAMs can outperform traditional methods, which rely only on a particular sensor, such as a Lidar, even with lower costs. VSLAM approaches utilize different camera types (e.g., monocular, stereo, and RGB-D), have been tested on various datasets (e.g., KITTI, TUM RGB-D, and EuRoC) and in dissimilar environments (e.g., indoors and outdoors), and employ multiple algorithms and methodologies to have a better understanding of the environment. The mentioned variations have made this topic popular for researchers and resulted in a wide range of VSLAMs methodologies. In this regard, the primary intent of this survey is to present the recent advances in VSLAM systems, along with discussing the existing challenges and trends. We have given an in-depth literature survey of forty-five impactful papers published in the domain of VSLAMs. We have classified these manuscripts by different characteristics, including the novelty domain, objectives, employed algorithms, and semantic level. We also discuss the current trends and future directions that may help researchers investigate them.

==> temp.tex <==
% ------------- Summary of Papers -----------------

% ----------------------- VSLAM Approaches ---------------------
% xiao2019dynamic (Dynamic-SLAM)
The Dynamic-SLAM framework was proposed by authors in [x] and leverages deep learning for accurate pose prediction and suitable environment comprehension. As part of a semantic level module for optimized visual odometry, the authors employed a CNN to identify moving objects in the environment, which helped them lower the pose estimate error brought on by improper feature matching. Additionally, dynamic-SLAM is outfitted with a selective tracking module to ignore dynamic locations in the scene and a missed feature corrective algorithm for speed invariance in adjacent frames. Their real-time feature-based framework is built on the base of ORB-SLAM 2.0 and works with monocular cameras. Dynamic-SLAM could outperform ORB-SLAM 2.0 in feature extraction and has been tested on a UGV and various datasets, including TUM RGB-D, KITTI, and authors generated. Despite the excellent results, this system requires huge computational costs and faces the risk of misclassifying dynamic and static objects due to a limited number of defined semantic classes.

% sumikura2019openvslam (OpenVSLAM)
The authors [x] introduce a highly customizable open-source VSLAM software, OpenVSLAM, that aims to be easily adapted, improved, and called by other third-party programs. Their indirect approach is compatible with various camera types, including monocular, stereo, and RGB-D cameras, and can store created maps and reuse previously generated map databases. OpenVSLAM contains three main components: tracking, mapping, and global optimization. Due to a more robust ORB feature extractor module, this approach outperforms ORB-SLAM and ORB-SLAM 2.0 in tracking accuracy and time. They have tested their system on the EuRoC MAV dataset with indoor instances. Despite the good features of OpenVSLAM, the contributors terminated the release of their software due to code similarities concerns that violate ORB-SLAM 2.0 copyright.
https://github.com/xdspacelab/openvslam

% kerl2013dense
Authors in [x] proposed a real-time dense SLAM method for RGB-D cameras, improving their previous technique, kerl2013robust, by minimizing the photometric and geometric errors between two images for camera motion detection. Their keyframe-based approach extends Pose-SLAM (ila2009information), combines dense visual odometry features, and can efficiently exploit the information from camera frames for a robust camera motion estimation. For loop closure detection and drift avoidance, they use an entropy-based method for measuring the similarity of the keyframes. According to the experiments performed on the TUM RGB-D dataset indoor instances, their method can perform well in scenes with low texture information. However, their system needs improvement regarding keyframe selection quality and loop closure detection.
https://vision.in.tum.de/data/software/dvo

% ila2009information (Pose-SLAM, referred in kerl2013dense) -------------> Needs improvement
The map is represented as a graph in Pose SLAM, with the vertices representing absolute sensor poses and the edges representing relative sensor transformations.

% zhou2015structslam (StructSLAM)
Zhou et al. [x] presented a novel idea of using building structure lines as practical features instead of utilizing element points to estimate the correct camera pose and build the map of the surroundings. As structure lines are associated with dominant directions and encode global orientation information, the camera's heading will be constrained, and the orientation errors will reduce, leading to improved estimated trajectories. The mentioned approach, titled StructSLAM, is a 6-DoF VSLAM method that works in low-feature and featureless environments. StructSLAM uses the Extended Kalman Filter (EKF) algorithm for estimating variables based on the existing directions in the world frame. For experiments, the authors tested their method on a set of generated sequential images and RAWSEEDS 2009's indoor scenes dataset.

% yu2018ds (DS-SLAM)
Yu et al. [x] proposed a VSLAM system titled DS-SLAM that can be employed in dynamic environments and provide semantic-level data when building the map. Their approach is based on ORB-SLAM 2.0 and contains five threads: tracking, semantic segmentation, local mapping, loop closing, and dense semantic map creation, making it a robust but computationally intensive system. DS-SLAM uses a real-time semantic segmentation network called SegNet and applies the Optical Flow algorithm to discard dynamic objects before the pose estimation process and improve localization accuracy. It also builds dense semantic 3D octrees-based maps for higher-level robotics tasks. The system works with RGB-D cameras and has been tested on the TUM RGB-D dataset and in a real-world scenario. Despite DS-SLAM's high accuracy in localization, there is a chance of semantically segmentation limitation.
https://github.com/ivipsourcecode/DS-SLAM

% pumarola2017pl (PL-SLAM)
Pumarola et al. [x] presented Point and Line SLAM (PL-SLAM), a VSLAM system built upon ORB-SLAM designed for non-dynamic low texture environments that simultaneously combines line and point features for more satisfactory pose estimation. The significant advantage of their approach is the ability to work in environments with a small number of feature points. PL-SLAM is equipped with a tracking thread for keyframe addition based on the predicted camera position, a local mapping thread for appending new keyframes data into the map, and a loop closing thread for identifying and correcting loops. It also contains a line-based map initialization method that estimates camera pose and 3D map from line correspondences in three consecutive images. Researchers tested their approach on TUM RGB-D and a generated dataset. The disadvantage of PL-SLAM is the computational cost and the essence of using other geometric primitives, e.g., planes, for a more robust accuracy.
https://github.com/HarborC/PL-SLAM

% bloesch2018codeslam (CodeSLAM)
Bloesch et al. proposed a direct approach titled Code-SLAM that provides a compact and dense representation of the scene geometry. Their SLAM system is an improved version of PTAM (klein2007parallel) and works only with monocular cameras. They used a CNN trained on intensity images of the SceneNet RGB-D dataset to decompose intensity images into convolutional features and feed them to a depth auto-encoder. Code-SLAM has been tested on the indoor instances of the EuRoC dataset and could achieve robust results in terms of performance and accuracy.
https://github.com/silviutroscot/CodeSLAM

% cui2019sof (SOF-SLAM)
Cui and Ma [x] proposed Semantic Optical Flow SLAM (SOF-SLAM), an indirect VSLAM system built upon the RGB-D mode of ORB-SLAM 2.0 and works in highly dynamic conditions. Their method uses a dynamic feature detection module called Semantic Optical Flow that extracts and skips the changing characteristics hidden in semantic and geometry information provided by ORB feature extraction. Using SegNet's pixel-wise semantic segmentation module, SOF-SLAM provides reliable camera position and environment reports. Experimental results on the TUM RGB-D dataset and real-world environments showed that SOF-SLAM works better than ORB-SLAM 2.0 in highly dynamic scenarios. The weakness of SOF-SLAM is the inefficient process of non-static feature detection and relying on only two consecutive frames for this purpose.

% zou2012coslam (CoSLAM)
Zou and Tan [x] proposed a VSLAM system called CoSLAM that utilizes multiple independent cameras mounted on different platforms for a more robust map-building process. Their system clusters cameras into distinct groups regarding their view overlap and facilitates the 3D reconstruction of dynamic points by combining intra- and inter- camera pose estimation and mapping. It uses Kanade-Lucas-Tomasi (KLT) algorithm for feature detection and tracking. CoSLAM works in indoor and outdoor static and highly dynamic environments where relative positions and orientations may change over time. It has been evaluated on a generated dataset with the scalability of twelve cameras. The major drawback of their approach is the need for powerful hardware to process multiple camera outputs, and increasing the number of cameras results in higher computational costs. Despite the benefits of CoSLAM, one of the challenging factors is synchronizing the cameras.
https://github.com/danping/CoSLAM

% li2021dp (DP-SLAM)
Authors in [x] proposed a feature-based VSLAM method called DP-SLAM that uses a Bayesian probability propagation model based on the likelihood of the keypoints extracted from moving objects for real-time dynamic object removal. Utilizing the moving probability propagation algorithm and iteratively updating the probability enables DP-SLAM to overcome the deviation of geometry constraints and semantic data for effective visual odometry. In their approach, they performed pre-processing to remove data associated with moving objects and fill the background section occluded by them with recognized static points across several frames to improve the mapping performance in a dynamic environment. DP-SLAM is integrated with ORB-SLAM 2.0 and has been tested on the TUM RGB-D dataset. Despite the accurate results, the system only works in sparse VSLAMs and faces high computational costs because of the iterative probability updater module.

% xu2020edge (edgeSLAM)
Xu et al. [x] proposed edgeSLAM, an edge-assisted semantic VSLAM system for mobile and for resource-constrained devices that works in real-time. Instead of using heavy threads, edgeSLAM uses a set of fine-grained modules to be employed by the edge server and the connected mobile devices. It is also equipped with a semantic segmentation module based on the Mask-RCNN algorithm. The authors implemented their approach on an edge server with different commercial mobile devices, including smartphones and development boards. As a novel computation offloading strategy, they adopted system parameters to various network bandwidth and latency conditions and prevented redundant computation by reusing the object segmentation results. For experimental setups, edgeSLAM has been tested on monocular vision instances of TUM RGB-D, KITTI, and the dataset generated by the authors.

% li2020dxslam (DXSLAM)
Li et al [x] proposed a publicly available VSLAM system named DXSLAM that uses deep learning to detect SuperPoint-like keypoints and generate both the keypoints and images' general descriptors. They trained HF-NET, a state-of-the-art deep CNN, to extract local and global features per frame and generate frame- and keypoint-based descriptions. Additionally, they trained a visual vocabulary of local features using the offline BoW method for accurate loop closure detection. Their approach achieves a higher accuracy with a lower computational cost compared to BoW methods. DXSLAM is compatible with modern CPUs and runs in real-time without the aid of GPU. In dynamic environments, it has a strong capability to resist dynamic changes, even though such features are not explicitly addressed. DXSLAM has been tested on TUM RGB-D and OpenLORIS-Scene datasets and both indoor and outdoor images and could achieve more accurate results than ORB-SLAM 2.0 and DS-SLAM. However, the major disadvantages of this method are complex architecture for feature extraction and incorporating deep features into an old SLAM framework.
https://github.com/ivipsourcecode/dxslam

% vidal2018ultimate (Ultimate SLAM)
Vidal et al. [x] proposed the idea of combining events, camera frames, and IMU in parallel setups for robust pose estimation in high-speed scenarios. Their method, Ultimate SLAM, is built on a keyframe-based nonlinear optimization pipeline for visual odometry in event cameras [x]. The pipeline processes events in overlapping spatio-temporal windows and uses the current camera motion to align them, resulting in an accurate camera pose estimation. They use the FAST corner detector and Lucas-Kanade tracking algorithm for feature detection and tracking, respectively. Ultimate SLAM works in various dynamic environments with varying illumination conditions and bypasses motion blur issues caused by high-speed activity. Experimental results on the "Event Camera Dataset" showed the effectiveness of this VSLAM approach compared to other event-only and standard camera setups. The authors also tested their system on an autonomous quadrotor equipped with an event camera to demonstrate the ability to handle unreachable flight scenarios with traditional VO platforms. The major challenge in Ultimate SLAM is the synchronization of events with standard frame outputs.
% https://github.com/uzh-rpg/rpg_ultimate_slam_open

% zhu2021camvox (CamVox)
Zhu et al. [x] proposed an indirect lidar-assisted VSLAM named CamVox that shows robust performance and accuracy while keeping it a low-cost solution. Their system utilizes ORB SLAM 2.0 and fuses the unique features provided by Livox lidars as the high-end depth sensors with the RGB-D camera outputs. CamVox demonstrated a long-range outdoor capability and accurate measurements. The authors also used an IMU for correcting the non-repeating scanned points and synchronization. Another contribution of their work is proposing an automatic lidar-camera calibration technique that works in uncontrolled settings. According to the real-world experiments on a robot platform, CamVox shows a real-time performance while processing the environment.
https://github.com/ISEE-Technology/CamVox

% cheng2019improving
Cheng et al. [x] proposed a VSLAM system that uses the Optical Flow algorithm to distinguish and eliminate dynamic feature points. They have used the structure of the ORB-SLAM pipeline and fed it with the static feature points obtained by standard monocular camera outputs for accurate pose estimation. The mentioned system contains ego-motion analysis and optical flow-based detection modules and works in featureless scenarios by sorting optical flow values and using them for feature detection. Experimental outcomes on the TUM dataset showed that the proposed system works fine in dynamic indoor conditions. However, the system is configured using an offline threshold for motion analysis, making it challenging for various dynamic environment conditions.

% li2020textslam (TextSLAM)
Li et al. [x] proposed TextSLAM, a text-based VSLAM system that integrates text objects extracted by the FAST corner detection algorithm from the scene into the SLAM pipeline. Texts are rich in textures, patterns, and semantic meanings, and employing them to generate high-quality 3D text maps leads to better performance. TextSLAM utilizes texts as good visual fiducial markers, parametrizes them when first detected in a frame, and projects the 3D text object onto the target image to find it again. The camera pose will be estimated by calculating the photometric error by comparing the projected and observed text. They also raised a novel three-variable parameterization method for instantaneous text features initialization. Experiments in indoor and outdoor environments using a monocular camera on a dataset generated by the authors showed high accuracy outcomes. The main challenges of TextSLAM are operating in text-less environments, reading small texts, and requiring storage of huge text dictionaries.

% yang2020multi
Yang et al. [x] proposed a panoramic vision VSLAM technique based on multi-camera cooperation for complex off-road environments. Their method can provide independence and information sharing for each camera to improve the performance of the VSLAM system under various challenging scenarios, including illumination, occlusion, and sparsity of textures. Thus, they extract ORB features from the cameras overlapping fields of view to calculate the matching range and estimate the camera pose. They also used a deep learning method based on a modified CNN to represent aggregated image features into a fixed-length vector and detect repeated scenes for an efficient loop closure detection. The authors utilized a dataset generated with a panoramic camera and an integrated navigation system for the experiment.

% xu2019occupancy
Xu et al. [x] proposed an indirect VSLAM system built upon a modified ORB SLAM that enables high-accuracy localization and user interaction using the Occupancy Grid Mapping (OGM) method and a new 2D mapping module. Using the OGM, their system can build the environment map represented as an evenly spaced field of variables showing the presence of an obstacle. Another contribution of their work is enabling path planning and continuous and real-time navigation. Their system works with RGB-D cameras and indoor GPS-denied environments, according to the experimental analysis of a generated dataset. However, their method cannot perform well in complex and dynamic settings and faces challenges in correctly matching the features in corridors and feature-less scenarios.

% bultmann2019stereo (DQV-SLAM)
Authors in [x] proposed Dual Quaternion Visual SLAM (DQV-SLAM), a VSLAM framework for stereo-vision cameras that uses a general Bayesian framework for 6-DoF pose estimation. Their system performs progressive Bayes updates to avoid linearization of the nonlinear spatial transformation group. DQV-SLAM uses ORB features to make point clouds of maps and optical flow to ensure robust data association in dynamic scenarios. This approach is reliable for accurately estimating the experiment outcomes on KITTI and EuRoC datasets. However, this approach is computationally intensive in sampling approximation-based filtering and lacks probabilistic interpretation for stochastic modeling of the poses.

% li2021deep
Li et al. [x] proposed a deep learning-based real-time VSLAM approach for extracting feature points in complex scenes. The method is a multi-task CNN for feature extraction with self-supervision abilities and can run on a GPU while supporting 3D dense map construction. The CNN output is binary code strings with a fix-length of 256, which enables it to be replaced by traditional feature point detectors, such as ORB. It consists of three threads for robust and real-time performance in dynamic scenes, including tracking, local mapping, and loop closing. They used ORB-SLAM 2.0 as their baseline and developed a system that promotes monocular and RGB-D cameras. The authors tested their approach on the TUM dataset and two generated datasets collected in a corridor and an office using a Kinect camera for the experiments.

% ferrera2021ov (OV2SLAM)
Ferrera et al. [x] designed {OV$^{2}$SLAM}, a VSLAM system to close the gap between real-time capability, accuracy, and robustness that works with monocular and stereo-vision cameras. Their approach reduces the computational load by limiting the extraction of features to keyframes and tracking them in subsequent frames by minimizing the photo-metric errors. In this regard, {OV$^{2}$SLAM} is a hybrid approach that combines the characteristics of the algorithms in direct and indirect categories. It contains four threads: front-end, mapping, state optimization, and loop closing. Experiments in indoor and outdoor environments using widely used benchmarking datasets such as EuRoC, KITTI, and TartanAir showed that {OV$^{2}$SLAM} outperforms some well-known approaches in terms of performance and accuracy.
https://github.com/ov2slam/ov2slam

% bruno2021lift (LIFT-SLAM)
Bruno and Colombini [x] proposed LIFT-SLAM, which integrates deep learning-based feature descriptors with the traditional geometry-based VSLAM systems. They extended the conventional VSLAM pipeline of the ORB-SLAM system and used a CNN to extract features from images and use the learned features to obtain more dense and accurate matches. LIFT-SLAM utilizes transfer learning and fine-tuning of a Learned Invariant Feature Transform (LIFT) deep neural network for detection, description, and orientation estimation purposes. Their system works on monocular cameras. Experiments on Indoor and Outdoor instances of KITTI and EuRoC MAV datasets showed that LIFT-SLAM surpasses traditional feature-based and deep learning-based VSLAM systems in terms of accuracy. The primary drawbacks of LIFT-SLAM are its computationally intensive pipeline and unoptimized CNN architecture that results in almost real-time performance.

% dong2019pair (Pair-Navi)
Dong et al. [x] proposed an indoor navigation system called Pair-Navi that re-uses a previously traced path by an agent for future use by other agents. With this, a previous traveler named a leader records the trace information, including turnings and specific ambient properties, and shares it with a later follower who needs to travel to the same destination. The trace information will be requested by and sent to the follower. The leader contains visual odometry and trajectory construction modules, while the follower locates its relative location to the reference trace by a relocalization module. Pair-Navi supports Peer-to-Peer (P2P) mode and performs in real-time. The system uses a Mask Region-based CNN (Mask R-CNN) to identify and delete dynamic objects from the video feature set. They tested Pair-Navi on a set of generated datasets and several smartphones for the experiments.

% lim2021avoiding
Lim et al. [x] introduced a degeneracy avoidance algorithm for monocular point- and line-based VLSAM systems. Their system utilizes both features to understand the environment better. Another contribution of their method is a robust Optical Flow-based line tracking module that extracts line features, ignores short lines in each frame, and matches the previously detected lines. They tested their system on EuRoC MAV dataset samples to prove the validity of their method and could achieve better results than the standard point-based approaches. Despite the robust results, the system lacks an adaptive algorithm to find the proper optimization factors.

% nguyen2020tightly
Nguyen et al. [x] proposed a tightly-coupled monocular camera and Ultra-Wideband (UWB) ranging sensors for VSLAM. Their method makes a map 
by combining feature-based (visible) and feature-less (UWB) landmarks. UWB works robustly when facing multi-path effects in cluttered environments. Their indirect approach is based on ORB-SLAM and uses ORB features for pose estimation. They tested their system on a generated dataset with hand-carried movements emulating an employed aerial robot for the experiment. One of the challenges here is the synchronization of the camera and UWB sensor, which has been resolved using a new camera pose with its corresponding timestamp for each new image. However, the estimate in this approach is still of local type.

% munoz2020ucoslam (UcoSLAM)
Muñoz-Salinas and Medina-Carnicer proposed a method titled UcoSLAM [x] that outperforms traditional VSLAM systems by fusing natural and artificial landmarks and automatically determining the scale of the environment using fiducial markers. The primary motivation of UcoSLAM is to overcome instability, repetitiveness, and insufficient characteristics of natural landmarks for tracking. It can work in keypoints-only, markers-only, and combined modes, making it available to work in markerless and featureless environments. UcoSLAM contains a tracking mode to find map correspondences and reprojection error optimization and a relocalization mode in case of tracking failure. It also includes a marker-based loop closure detection and feature description and can use any descriptors, such as ORB or FAST. Despite all the plus points of UcoSLAM, the system executes in multiple threads, making it a time-consuming approach.

% teed2021droid (Droid-SLAM)
Teed and Deng [x] proposed DROID-SLAM, a deep learning-based visual SLAM for monocular, stereo, and RGB-D cameras. They could achieve higher accuracy and robustness than well-known monocular and stereo track approaches. Their system works in real-time and consists of front-end (for keyframe collection and graph optimization) and back-end (for bundle adjustment) threads. DROID-SLAM is trained with monocular camera instances and can use stereo and RGB-D inputs without the need to be trained again. The method is neither direct nor indirect, as it does not require any pre-processing for feature detection and matching and minimizes the projection error, similar to indirect methods. Each input image is processed by a feature extraction network, consisting of residual blocks and down-sampling layers to produce dense features. The system has been tested on well-known datasets, including TartanAir, EuRoC, and TUM RGB-D, and could achieve acceptable results.
https://github.com/princeton-vl/DROID-SLAM

% ma2016cpa (CPA-SLAM)
Ma et al. [x] proposed a direct VSLAM technique for RGB-D cameras titled  CPA-SLAM that uses planes for tracking and graph optimization. Their method consistently integrates frame-to-keyframe and frame-to-plane alignment. Another contribution of their work was introducing an image alignment method for tracking the camera concerning a reference keyframe and aligning the image with the planes. CPA-SLAM employs the keyframe data and searches for its corresponding small temporal and spatial distances for tracking. The system was analyzed on TUM RGB-D and ICL-NUIM datasets with indoor and outdoor scenes, and the real-time performance of their tracking system was tested in with- and without-plane scenarios. However, the major weakness of their work is supporting the limited geometric shape, i.e., planes.

% schlegel2018proslam (ProSLAM)
Schlegel, Colosi, and Grisetti [x] proposed a lightweight feature-based VSLAM framework titled ProSLAM for stereo camera setups that provides results comparable to state-of-the-art methods. Their method contains four modules, including a triangulation module for producing 3D points plus corresponding feature descriptors, an incremental motion estimation module for processing a pair of frames to obtain the current position, a map management module for generating local maps, and a re-localization module for updating the world map based on the similarities of local maps. ProSLAM uses a minimal set of well-known libraries for an easily implemented system and obtains the 3D position of the points using a single thread. It creates a local map of the environment using the landmarks detected in a nearby region. According to the experiments on KITTI and EuRoC datasets, their approach could achieve robust results. However, ProSLAM shows weakness in rotation estimation and does not contain any bundle adjustment module.
% https://gitlab.com/srrg-software/srrg_proslam

% urban2016multicol (MultiCol-SLAM)
MultiCol-SLAM, an open-source VSLAM framework that supports multi-camera configurations, was presented by Urban and Hinz [x]. They use their previously created model, MultiCol, to enhance ORB-SLAM utilizing a keyframe-based process that supports multiple fisheye cameras. They added a Multi-Keyframes (MKFs) processing module to ORB-SLAM, which gathers numerous fisheye camera images and turns them into keyframes. They also proposed the idea of multi-camera loop closing, in which loop closures from MKFs are detected by a loop closing thread. They put MultiCol-SLAM to the test on a produced dataset to determine how using several fisheye cameras affected the accuracy, tracking, and performance of the ORB-SLAM architecture. Although their method operates in real-time, it requires a significant amount of computer power because several threads must run simultaneously.
% https://github.com/urbste/MultiCol-SLAM

% wang2017deepvo (DeepVO)
Wang et al. [X] proposed DeepVO, an end-to-end VO framework using a Deep Recurrent CNN (RCNN) architecture for monocular setups. Their method can directly infer poses from color frames and utilize deep learning to learn appropriate features automatically and model sequential dynamics and relations. The architecture of DeepVO contains a CNN titled FlowNet for computing optical flow from sequential frames and two Long-Short Term Memory (LSTM) layers for estimating the temporal changes based on the feed provided by the CNN. Using the combination of CNN and RNN, the framework can simultaneously extract visual features and perform sequential modeling. DeepVO cannot be used as a replacement for traditional geometry-based VO methods, but it can incorporate geometry with the knowledge models learned for an improved VO. They tested their framework on the KITTI dataset and could achieve satisfactory accuracy in pose estimation.
% http://senwang.gitlab.io/DeepVO/

% parisotto2018global
Parisotto et al. [X] proposed an end-to-end system similar to DeepVO that employs a Neural Graph Optimization (NGO) stage instead of LSTMs. Their method utilizes a loop closure detection and correction method based on the temporally different poses. NGO jointly optimizes the aggregated predictions produced by convolutional layers of local pose estimation modules and provides global pose estimates using a pair of attention-optimization processes. They tested their approach on 2D and 3D mazes and could achieve appropriate accuracy and performance compared to DeepVO. However, the mentioned method needs to be attached to a SLAM framework to provide the relocalization signals.

% nguyen2021viral
Authors in [x] proposed a multi-modal SLAM system titled VIRAL (Visual-Inertial-Ranging-Lidar) SLAM that couples camera, lidar, IMU, and UWB for accurate enactment. They also presented a map-matching marginalization scheme for visual features based on the local map constructed from lidar point clouds. The visual components are extracted and tracked using Binary Robust Independent Elementary Features (BRIEF) algorithm. The framework also contains a synchronization scheme and trigger for the utilized sensors. They tested their approach on simulation environments and a generated dataset by the authors titled NTU VIRAL [x] that contains data produced by the camera, lidar, IMU, and UWB sensors. However, their approach is computationally intensive due to handling synchronization, multi-threading, and sensor conflict resolution.

% munoz2019spm
Muñoz-Salinas et al. [x] proposed a system to reconstruct a large-scale indoor environment map using artificial squared planar markers. Given at least two markers visible in each image, their real-time SPM-SLAM system can overcome the ambiguity problem. Their method performs a global optimization when there are no more frames to be processed. They tested SPM-SLAM based on the accuracy in correctly estimating markers and frame poses and could achieve better results than popular approaches, including ORB-SLAM 2.0 and LSD-SLAM. For evaluation, they generated a dataset containing video sequences of markers placed in two rooms connected by a door. Although their technique is cost-effective, it operates only when many planar markers are placed in the environment, while at least two of them are visible for the marker connection recognition task. Moreover, the ability of their framework to handle dynamic changes in the scene is not measured.

% czarnowski2020deepfactors
Czarnowski et al. [x] proposed DeepFactors, one of the most comprehensive VSLAM frameworks for densely reconstructing the environment map using monocular cameras. Their real-time method performs joint optimization of the pose and depth, utilizes probabilistic data, and incorporates both learned and model-based approaches for a more robust map reconstruction. The authors modified the CodeSLAM framework and added missing components such as local/global loop detection. Hence, the system contains a U-Net for extracting features from the input image and a Variational Auto-Encoder (VAE) for learning optimizable features. The system is trained on approximately 1.4 million images of ScanNet [x] and tested on ICL-NUIM and TUM RGB-D datasets. DeepFactors improves the idea of the CodeSLAM framework and focuses on code optimization in traditional SLAM pipelines. However, due to the computational costs of the modules, this approach requires employing GPUs to guarantee real-time performance.
% https://github.com/jczarnowski/DeepFactors

% gomez2019pl
Gomez-Ojeda et al. [x] proposed a VSLAM approach titled PL-SLAM (different from the framework with the same name by Pumarola et al.) that utilizes points and lines in stereo vision cameras for creating an unseen map. Their indirect method leverages segments obtained from points and lines in all VSLAM modules and merges them with visual features extracted from consecutive frames. In PL-SLAM, points and line segments are extracted using ORB and Line Segment Detector (LSD) methods and tracked in successive stereo frames. The 3D camera motion is computed by minimizing the projection errors. The authors tested PL-SLAM on EuRoC and KITTI datasets and could outperform the stereo version of ORB-SLAM 2.0 in terms of performance. One of the main drawbacks of PL-SLAM is the computational time required for the feature tracking module and considering all structural lines to extract information about the environment.
% https://github.com/rubengooj/pl-slam

% ben2020edge
Ben Ali et al. [x] proposed the idea of utilizing edge computing to enable offloading of resource-intensive tasks to the cloud reducing the computational overhead on the robot. In their indirect framework, titled Edge-SLAM, they modified the architecture of ORB-SLAM 2.0 by keeping the tracking module on the robot and assigning the rest to the edge. Hence, the system sustains a local and global map by dividing the VSLAM pipeline between the robot and the edge apparatus. They could achieve proper performance in limited resource conditions without affecting accuracy. They used the TUM RGB-D dataset and two different mobile devices to generate a custom indoor environment dataset using RGB-D cameras for evaluation. However, one of their approach's drawbacks is the architecture's complexity due to the decoupling of various SLAM modules. Another setback is that their system works only in short-term settings, and utilizing Edge-SLAM in long-term scenarios (e.g., multiple days) would face performance degradation.
% https://github.com/droneslab/edgeslam

% liu2019dms
DMS-SLAM [x] is another VSLAM approach for indoor and outdoor dynamic environments that supports monocular, stereo, and RGB-D visual sensors. The system uses the Grid-based Motion Statistics (GMS) feature matching and sliding window algorithms to detect static feature points. DMS-SLAM is built upon ORB-SLAM 2.0 system and only tracks the static features identified by the ORB algorithm. The authors tested their proposed method on TUM RGB-D and KITTI datasets and could achieve outperforming results compared to the state-of-the-art VSLAM systems. Moreover, DMS-SLAM performs faster than the original ORB-SLAM 2.0 due to removing the feature points on the dynamic objects in the tracking stage. Despite the mentioned advantages, the proposed method faces challenges in fast-motion scenarios, low-texture scenes, and highly dynamic environments.
% GMS: bian2017gms

% bavle2020vps
Bavle et al. [x] proposed VPS-SLAM, a lightweight graph-based VSLAM framework executable for aerial robotic platforms. Their real-time system integrates visual/visual-inertial odometry with geometrical information and various object detection methods for pose estimation and creating the semantic map of the environment. VPS-SLAM uses low-level features along with IMU measurements for robot state prediction and high-level planar information to correct pose estimation and reconstruct sparse semantic maps. The system uses the lightweight version of You Only Look Once (YOLOv2) trained on the COCO dataset for object detection due to its real-time and computationally efficient performance. The obtained bounding boxes of the object detector will then be used for semantic segmentation and graph. They used a hand-held camera setup and an aerial robotic platform with an RGB-D camera installed for evaluation. They also tested their approach on indoor instances of the TUM RGB-D dataset and could achieve results comparable to popular VSLAM techniques. However, their system can employ a limited number of objects (e.g., chairs, books, and laptops) to create a semantic map of the environment.
% YOLOv2: redmon2017yolo9000
% COCO: lin2014microsoft
% https://github.com/hridaybavle/semantic_slam

% naveed2022deep
Naveed et al. [X] proposed a deep learning-based VSLAM approach with a reliable and consistent tracking module, even on routes with extreme turns. Their method employed a deep reinforcement learning network trained on realistic simulators that outperformed several handcrafted VSLAMs. Moreover, they could perform proper generalization across real-world indoor and outdoor settings and introduced a benchmark for active VSLAM evaluation. Their used ORB-SLAM as the base system that receives the optimal path data generated by the network's path planner. For evaluation, they created a dataset containing thirty real-world navigation episodes in challenging and textureless scenarios. It should be noted that their system failed in particular scenarios due to improper training.

% peng2022rwt
Authors in [x] proposed a deep feature matching-based VSLAM framework for weak-textured environments, titled RWT-SLAM. Their system is built upon ORB-SLAM and feeds it with the feature masks provided by an improved version of the LoFTR [Y] for local image feature matching. Coarse-level and fine-level descriptors are extracted using a CNN and the LoFTR algorithm, respectively. RWT-SLAM is evaluated on TUM RGB-D and OpenLORIS-Scene datasets and a real-world dataset collected by the authors. However, despite the robust feature matching results and performance, their system is computationally intensive.
% LoFTR: sun2021loftr

% steenbeek2022cnn
Steenbeek and Nex in [X] proposed a real-time VSLAM method that employs a CNN for proper scene understanding and map reconstruction. Their system uses monocular camera streams from a UAV during the flight and leverages depth-estimating neural networks for robust performance. The mentioned approach is based on ORB-SLAM 2.0 and utilizes visual features obtained from indoor settings. Further, the CNN is trained on more than 48,000 indoor samples and uses the pose, space depth, and RGB inputs for scale/depth estimation. The system was evaluated on the TUM RGB-D dataset and a real-world test with a drone, showing improved accuracy in pose estimation.
However, the system requires both CPU and GPU resources for real-time performance and faces issues in texture-less scenarios. Additionally, the quality of the generated point clouds is low.

% tseng2022real
Tseng et al. [x] proposed a real-time indoor VSLAM approach that requires a low-cost setup. They also introduced a method to estimate the number of frames and visual features in each frame needed for an acceptable localization accuracy. Their system is built upon the OpenVSLAM framework and employs it for real-world emergency scenarios, such as finding access to particular targets. By acquiring the feature map of the scene, the system utilizes Efficient Perspective-n-Point (EPnP) and RANdom SAmple Consensus (RANSAC) algorithms for accurate pose estimation. According to the evaluations done in a building, their system can provide appropriate results in challenging illumination conditions.

% bonetto2022irotate
iRotate, an active VSLAM approach for omnidirectional robots with RGB-D cameras that generates control commands for localization and mapping, is proposed by Bonetto et al. in [X]. It also employs a module for detecting the presence of obstacles in the camera's field of view. The main goal of iRotate is to reduce the distance the robot traverses to map the environment by providing the observation coverage of previously unseen areas and already visited locations. The mentioned approach employs a graph-feature-based VSLAM framework as the backend. By presenting comparisons in simulation and on a real 3-wheel omnidirectional robot, they could achieve results comparable to state-of-the-art VSLAM techniques. However, the major weakness of their method is that the robot might face start-stop cases in which the local paths are replanned.
% https://github.com/eliabntt/irotate_active_slam

% 
Yang et al. [x] proposed another VSLAM approach that utilizes semantic segmentation network data combined with a motion consistency detection algorithm and geometric constraints for reconstructing the environment map. Their method is based on the RGB-D version of ORB-SLAM 2.0 and works fine in indoor and dynamic conditions. Using an improved ORB feature extraction algorithm, only the stable features remain in the scene, and the dynamic ones are ignored. Then, a static semantic map will be generated by combining the features with the semantic information. Evaluation results on Oxford and TUM RGB-D datasets showed that their approach could improve positioning accuracy and build semantic maps rich in information. However, their system might face challenges in corridors or areas containing less information.
